Phonon-mediated Hydrodynamic Transport in a Weyl Semimetal

We analyze from a microscopic point of view the feasibility of a hydrodynamic regime in a type-I Weyl semimetal driven by electron-electron interactions mediated by virtual phonons. Considering also the effects of of impurities and the absorption/emission of real phonons, the electric and thermal conductivities are derived. At temperatures $T$ above the Bloch-Gr\"uneisen temperature $T_\textrm{BG}$, virtual phonons behave similarly to real phonons, but the Lorenz ratio is modified by a constant prefactor dependent on the Fermi surface geometry. For temperatures below $T_\textrm{BG}$, processes that do not conserve chirality induce a $T^2$ dependence in the electric resistivity, opening a window where momentum-conserving interactions dominate transport signatures. We quantitatively discuss this hydrodynamic window and put it into context with recent experimental literature on the subject.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
